PEak: A Single Source of Truth for Hardware Design and Verification

Domain-specific languages for hardware can significantly enhance designer productivity, but sometimes at the cost of ease of verification. On the other hand, ISA specification languages are too static to be used during early stage design space exploration. We present PEak, an open-source hardware design and specification language, which aims to improve both design productivity and verification capability. PEak does this by providing a single source of truth for functional models, formal specifications, and RTL. PEak has been used in several academic projects, and PEak-generated RTL has been included in three fabricated hardware accelerators. In these projects, the formal capabilities of PEak were crucial for enabling both novel design space exploration techniques and automated compiler synthesis.

==> tex/background.tex <==
\section[bg]{Background}

Course Grain Reconfigurable Arrays (CGRA) \cite{cgra3,cgra1,cgra2} are a spatial architecture similar to FPGAs.  CGRAs are composed of Processor Elements (PEs), Memory tiles, and a configurable routing network that operates on a word-level. CGRAs trade off programmability with efficiency while being able to run a wide variety of applications making them a good choice for domain specific accelerators. Importantly, PEs and memory tiles can be \textit{specialized} to improve performance for application domains. % which is the basis for the DSE work using \peak.
